Identity Document and banknote security forensics: a survey

Counterfeiting and piracy are a form of theft that has been steadily growing in recent years. Banknotes and identity documents are two common objects of counterfeiting. Aiming to detect these counterfeits, the present survey covers a wide range of anti-counterfeiting security features, categorizing them into three components: security substrate, security inks and security printing. respectively. From the computer vision perspective, we present works in the literature covering these three categories. Other topics, such as history of counterfeiting, effects on society and document experts, counterfeiter types of attacks, trends among others are covered. Therefore, from non-experienced to professionals in security documents, can be introduced or deepen its knowledge in anti-counterfeiting measures.

==> futurework.tex <==
%\section{Future work}
%\label{section:future-work}

%To our knowledge we present in this work on of the most completes studies in anti-counterfeit features for security documents. One of the purposes of this work was to provide a reference for future researchers of the available datasets that they can work to continue developing new algorithms and techniques for counterfeit detection. Unfortunately the availability of ID and banknote datasets for this field continues to be an issue. Further study should be done in how it could be possible to create these datasets, without infrincting PII and copyright issues, to share for the research community and create a baseline of results. 

%In this work, we focus only in identity and banknotes. Both share similar anti-counterfeiting security features. A future line of work, would be doing the same analysis of tamper-evident labels, cheques, product authentication, stock certificates, postage stamps, etc. Then compare which of these objects has similar security features and which ones has easier available datasets. The objective would be two-fold. First study to possibility of using security detection algorithms of one object to the other. Second study if its possible to transfer knowledge between models trained in one printing security object dataset to the other. 

%Finally, the last objective of this work was to link each presented security feature with its corresponding research. The algorithm in each research publication, should preferably be designed with computer vision algorithms. This objective has not been entirely successful, due some of the presented security features it not clear there is a published research for them. 







==> url_images.tex <==
% Samples of security features
%https://www.any.hu/en/portfolio-items/valtozo-lezerkep/
